Investigating Lexical Sharing in Multilingual Machine Translation for Indian Languages

Multilingual language models have shown impressive cross-lingual transfer ability across a diverse set of languages and tasks. To improve the cross-lingual ability of these models, some strategies include transliteration and finer-grained segmentation into characters as opposed to subwords. In this work, we investigate lexical sharing in multilingual machine translation (MT) from Hindi, Gujarati, Nepali into English. We explore the trade-offs that exist in translation performance between data sampling and vocabulary size, and we explore whether transliteration is useful in encouraging cross-script generalisation. We also verify how the different settings generalise to unseen languages (Marathi and Bengali). We find that transliteration does not give pronounced improvements and our analysis suggests that our multilingual MT models trained on original scripts seem to already be robust to cross-script differences even for relatively low-resource languages

==> tabs/bilingual-baselines.tex <==
\begin{table}[!ht]
\centering\small
\setlength\tabcolsep{4pt}
\begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{6}{c}{\textbf{BLEU Score}}\\
    \midrule
    & \multicolumn{3}{c}{\textbf{Original}} & \multicolumn{3}{c}{\textbf{Transliterated}}\\
        \midrule
    & 5K & 8K & 10K & 5K & 8K & 10K\\
      \midrule
    Hi$\rightarrow$EN & 9.69 & 10.44 & \textbf{12.32} & - & - & -\\
    Ne$\rightarrow$EN & 2.10 & 2.33 & \textbf{2.37} & - & - & - \\
    Gu$\rightarrow$EN & 3.90 & 3.95 & \textbf{4.12} & 3.56 & 3.68 & \textbf{4.11}\\
    \bottomrule
  \end{tabular}
  \caption{BLEU scores for Bilingual MT models using shared BPE with vocabulary size $v$ in $\{ 5000, 8000, 10000\}$ }
  \label{tab:bilingual-baselines2}
\end{table}

==> tabs/data-sources.tex <==
\begin{table*}[!ht]
    \centering\small
    \begin{tabular}{llll}
    \toprule
     & Train & Dev & Test \\
    \midrule
    hi--en & Wikititles, HindEnCorp, IITB\footnotemark{} & WMT-dev14 & WMT-test14 \\
    ne--en & Bible,\footnotemark{} Ted2020,\footnotemark{} QED, GlobalVoices, GNOME, KDE  & Flores-dev & Flores-devtest \\
    gu--en & Bible, Wiki, Wikititles, Govin-clean, localisation & WMT-dev19 & WMT-test19 \\
    mr--en & Bible-UEDIN, cvit-pib, jw, PMI, Ted2020, Wikimatrix & Flores-dev & Flores-devtest \\
    be--en & alt, cvit-pib, JW, OpenSubtitles, PMI, Tanzil, Ted2020, Wikimatrix  & Flores-dev & Flores-devtest \\
    \bottomrule
    \end{tabular}
    \caption{The corpora used for each of the dataset splits for each language pair.}
    \label{tab:data:corpora}
\end{table*}



\addtocounter{footnote}{-2}
\footnotetext{\cite{kunchukuttan-etal-2018-iit}}
\addtocounter{footnote}{1}
\footnotetext{\cite{christodouloupoulos2015massively}}
%\addtocounter{footnote}{1}
\footnotetext{\cite{reimers-2020-multilingual-sentence-bert}}

==> tabs/data-stats.tex <==
\begin{table}[!ht]
    \centering\small
    \begin{tabular}{lrrr}
    \toprule
               & \multicolumn{3}{c}{\#sentences} \\
    Lang. pair & Train & Dev & Test \\
    \midrule
    % fi--en & 2,416,041 & 1,500 & 1,370 \\
    % et--en & 850,675 & 2,000 & 2,000 \\
    hi--en & 1,312,698 & 520 & 2,507 \\
    ne--en & 114,915 & 997 & 1,012 \\
    gu--en & 70,397 & 997 & 1,012\\
    \midrule
    \textit{mr--en} & 3,288,874 & 997 & 1,012 \\
    \textit{be--en} & 860,500 & 997 & 1,012 \\
    \bottomrule
    \end{tabular}
    \caption{Dataset sizes for each language pair.} %Top are languages used of training, bottom are languages used for few-shot and zero-shot analyses.}
    \label{tab:data:stats}
\end{table}

==> tabs/multilingual-results.tex <==
\begin{table*}[!ht]
\setlength\tabcolsep{4pt}
\centering\small
\begin{tabular}{lrrrrrrrrrrrr}
  %\begin{tabular}{lSSSSS}
    \toprule
    & \multicolumn{9}{c}{\textbf{Temperature}}\\
    &
      \multicolumn{3}{c}{Gu$\rightarrow$EN} &
      \multicolumn{3}{c}{Hi$\rightarrow$EN} &
      \multicolumn{3}{c}{Ne$\rightarrow$EN} \\
    \textbf{Vocab Size} & 1.2 & {1.5} & {1.8} & {1.2} & {1.5} & {1.8} & {1.2} & {1.5} & {1.8}  \\
      \midrule
          &  \multicolumn{9}{c}{\textit{Original}}\\
           \midrule
    char & \multicolumn{3}{c}{11.45} & \multicolumn{3}{c}{15.12} & \multicolumn{3}{c}{10.46} \\
    4K & 11.10 & 11.40 & \textbf{\textit{11.82}} & 15.03 & 14.14 & 14.34 & 11.12 & \textbf{11.85} & \textbf{12.10}\\
    8K & \textbf{11.46} & \textbf{11.69} & 11.58  & 15.01 & 14.60 & 14.66 & \textbf{\textit{12.52}} & 11.80 & 11.79 \\
    16K & 11.42 & 9.99 & 11.59 & 15.11 & 14.70  & \textbf{14.78}& 11.73 & 10.44 & 11.56 \\
    32K & 11.37 & 11.11 & 11.01& \textbf{\textit{15.32}} & \textbf{14.76} & 14.57 & 11.60 & 11.20 & 11.31\\
    \midrule
     & \multicolumn{9}{c}{\textit{Transliterated}}\\
     \midrule
    char & \multicolumn{3}{c}{\textit{11.82}} & \multicolumn{3}{c}{\textit{12.23}} & \multicolumn{3}{c}{10.12} \\
    4K & 11.17 & 11.30 & \textbf{11.62} & 11.33 & 11.24 & 11.53 & \textbf{12.23} & \textbf{12.52} & \textbf{\textit{12.56}}\\
    8K & 11.42 &\textbf{ 11.69 }& 11.36  &11.69 & 11.60 & \textbf{11.66} & 11.87 & 11.50 & 11.32 \\
    16K & 11.46 & 10.13 & 11.44 & \textbf{11.78} & \textbf{14.10} & 13.33 & 11.76 & 11.14 & 12.12 \\
    32K & \textbf{11.56} & 11.08 & 11.00 & 11.75 & 11.14 &  11.44 & 11.73 & 11.10 & 11.24\\
    
    \bottomrule
  \end{tabular}
  \caption{BLEU scores for multilingual translation model with original scripts and transliteration using BPE with temperature $t$ in $\{ 1.2,1.5,1.8 \}$ and vocabulary size $v$ in $\{ 16000,32000,48000 \}$. Bold represents best score for each temperature value, bold italics represents best score overall for BPE-models, italics represents best score overall. }
  \label{tab:multilingual-regular}
\end{table*}

==> tabs/zero-shot-transfer.tex <==
% \begin{table}[!ht]
% \setlength\tabcolsep{4pt}
% \centering\small
% \begin{tabular}{lrrrrrr}
%     \toprule
%     & \multicolumn{6}{c}{\textbf{Zero Shot Transfer}}\\
%     \midrule
%     & \multicolumn{6}{c}{\textit{Original}}\\
%     \midrule
%     & \multicolumn{3}{c}{\textbf{Be $\rightarrow$ En }} & \multicolumn{3}{c}{\textbf{Mr $\rightarrow$ En}}\\
%         \midrule
%     & 1.2 & 1.5 & 1.8 & 1.2 & 1.5 & 1.8 \\
%       \midrule
%    char & 2.53 & 2.61 & \textbf{2.64} & 4.23 & 4.54 & \textbf{4.86} \\
%    4K & 3.31 & 3.41 & \textit{\textbf{3.93}} & 4.89 & 5.12 & \textit{\textbf{5.56}} \\
%     8K & 3.50 & 3.55 & \textbf{3.67} & 4.45 & 4.83 & \textbf{5.32} \\
%     16K & 3.65 & 3.70 & \textbf{3.74} & 4.36 & 4.99 & \textbf{5.43}\\
%     32K & 3.21 & 3.25 & \textbf{3.26} & 4.11 & 4.35 & \textbf{5.40} \\
%     \midrule
%     & \multicolumn{6}{c}{\textit{Transliterated}}\\
%     \midrule
%     & \multicolumn{3}{c}{\textbf{Be $\rightarrow$ En }} & \multicolumn{3}{c}{\textbf{Mr $\rightarrow$ En}}\\
%         \midrule
%     & 1.2 & 1.5 & 1.8 & 1.2 & 1.5 & 1.8 \\
%       \midrule
%    char & 3.39 & 3.42 & \textbf{3.58} & 5.02 & 5.12 & \textbf{5.33} \\
%    4K & 3.68 & 3.79 & \textit{\textbf{4.23}} & 5.02 & 5.33 & \textit{\textbf{5.81}} \\
%     8K & 3.75 & 3.86 & \textbf{3.95} & 5.24 & 5.41 & \textbf{5.71} \\
%     16K & 3.77 & 3.83 & \textbf{3.99} & 5.15 & 5.62 & \textbf{5.68}\\
%     32K & 3.76 & 3.91 & \textbf{3.93} & 5.17 & 5.76 & \textbf{5.78} \\
%     \bottomrule
%   \end{tabular}
%   \caption{BLEU scores for zero-shot performance on English-Bengali and English-Marathi pairs using shared BPE with vocabulary size $v$ in $\{ 16000, 24000, 32000, 48000\}$ and char tokenisation using temperature $t$ in $\{ 1.2, 1.5, 1.8 \}$}
%   \label{tab:zeroshot-results}
% \end{table}
